Towards Nudging in BPM: A Human-Centric Approach for Sustainable Business Processes

Business Process Management (BPM) is mostly centered around finding technical solutions. Nudging is an approach from psychology and behavioral economics to guide people's behavior. In this paper, we show how nudging can be integrated into the different phases of the BPM lifecycle. Further, we outline how nudging can be an alternative strategy for more sustainable business processes. We show how the integration of nudging offers significant opportunities for process mining and business process management in general to be more human-centric. We also discuss challenges that come with the adoption of nudging.

==> 04-reseach-potential.tex <==
\section{Research potential of Nudging in Process Mining} 
\label{sec:research-potential}

\subsection{Opportunities}

\begin{itemize}
    \item Designing interventions in an effective way
    \item Better process conformance
    \item Allowing for better process redesign
    \item 
\end{itemize}

\subsection{Challenges}

\begin{itemize}
    \item Studying nudges in a controlled manner might be difficult, especially in design time
    \item 
\end{itemize}
	

